A Practical Mini-Course on Applied Holography

This is a collection of notes based on lectures given at IIT Madras in September 2019 and at IFT Madrid in November 2019. It is supposed to be a concise (and therefore not comprehensive) and pragmatic course on applied holography and especially the (basic) analytic and numerical techniques involved. The lectures are not focused on the large theoretical and fundamental background which can be found already in several places in the literature, but rather on concrete applications of Bottom-Up AdS-CFT to Hydrodynamics, QCD and Condensed Matter. The idea is to accompany the reader step by step through the various benchmark examples with a classmate attitude, providing details of the computations and open-source numerical codes in Mathematica, and sharing simple tricks and warnings collected during my research experience. At the end of this path, the reader will be in possess of all the fundamental skills and tools to learn by himself/herself more advanced techniques and to produce independent and novel research on the topic.

==> acronym.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acronyms}

Use the template \emph{acronym.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your list(s) of abbreviations or symbols.

Lists of abbreviations\index{acronyms, list of}, symbols\index{symbols, list of} and the like are easily formatted with the help of the Springer-enhanced \verb|description| environment.

\begin{description}[CABR]
\item[ABC]{Spelled-out abbreviation and definition}
\item[BABI]{Spelled-out abbreviation and definition}
\item[CABR]{Spelled-out abbreviation and definition}
\end{description}

==> dedication.tex <==

%%%%%%%%%%%%%%%%%%%%%%% dedic.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% sample dedication
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{dedication}
Use the template \emph{dedic.tex} together with the Springer document class SVMono for monograph-type books or SVMult for contributed volumes to style a quotation or a dedication\index{dedication} at the very beginning of your book
\end{dedication}






==> foreword.tex <==
%%%%%%%%%%%%%%%%%%%%%%foreword.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample foreword
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\foreword

%% Please have the foreword written here
Use the template \textit{foreword.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your foreword\index{foreword}. 

The foreword covers introductory remarks preceding the text of a book that are written by a \textit{person other than the author or editor} of the book. If applicable, the foreword precedes the preface which is written by the author or editor of the book.


\vspace{\baselineskip}
\begin{flushright}\noindent
Place, month year\hfill {\it Firstname  Surname}\\
\end{flushright}




==> part1.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{Part Title}

    
\end{partbacktext}

==> part2.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{Part Title}
\noindent Use the template \emph{part.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your part title page and, if desired, a short introductory text (maximum one page) on its verso page.

\end{partbacktext}

==> part3.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{Part Title}
\noindent Use the template \emph{part.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your part title page and, if desired, a short introductory text (maximum one page) on its verso page.

\end{partbacktext}

==> part4.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{Part Title}
\noindent Use the template \emph{part.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) to style your part title page and, if desired, a short introductory text (maximum one page) on its verso page.

\end{partbacktext}

==> references.tex <==
\begin{thebibliography}{100}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi:\discretionary{}{}{}#1}\else
  \providecommand{\doi}{doi:\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem{McGreevy:2016myw}
J.~McGreevy,
\newblock \emph{{TASI 2015 Lectures on Quantum Matter (with a View Toward
  Holographic Duality)}},
\newblock In \emph{{Proceedings, Theoretical Advanced Study Institute in
  Elementary Particle Physics: New Frontiers in Fields and Strings (TASI 2015):
  Boulder, CO, USA, June 1-26, 2015}}, pp. 215--296,
\newblock \doi{10.1142/9789813149441_0004} (2017), \eprint{1606.08953}.

\bibitem{McGreevy:2009xe}
J.~McGreevy,
\newblock \emph{{Holographic duality with a view toward many-body physics}},
\newblock Adv. High Energy Phys. \textbf{2010}, 723105 (2010),
\newblock \doi{10.1155/2010/723105},
\newblock \eprint{0909.0518}.

\bibitem{Nastase:2007kj}
H.~Nastase,
\newblock \emph{{Introduction to AdS-CFT}}  (2007),
\newblock \eprint{0712.0689}.

\bibitem{Ramallo:2013bua}
A.~V. Ramallo,
\newblock \emph{{Introduction to the AdS/CFT correspondence}},
\newblock Springer Proc. Phys. \textbf{161}, 411 (2015),
\newblock \doi{10.1007/978-3-319-12238-0_10},
\newblock \eprint{1310.4319}.

\bibitem{Ammon:2015:GDF:2834415}
M.~Ammon and J.~Erdmenger,
\newblock \emph{Gauge/Gravity Duality: Foundations and Applications},
\newblock Cambridge University Press, New York, NY, USA, 1st edn.,
\newblock ISBN 1107010349, 9781107010345 (2015).

\bibitem{Aharony:1999ti}
O.~Aharony, S.~S. Gubser, J.~M. Maldacena, H.~Ooguri and Y.~Oz,
\newblock \emph{{Large N field theories, string theory and gravity}},
\newblock Phys. Rept. \textbf{323}, 183 (2000),
\newblock \doi{10.1016/S0370-1573(99)00083-6},
\newblock \eprint{hep-th/9905111}.

\bibitem{CasalderreySolana:2011us}
J.~Casalderrey-Solana, H.~Liu, D.~Mateos, K.~Rajagopal and U.~A. Wiedemann,
\newblock \emph{{Gauge/String Duality, Hot QCD and Heavy Ion Collisions}}
  (2011),
\newblock \doi{10.1017/CBO9781139136747},
\newblock \eprint{1101.0618}.

\bibitem{Zaffaroni_2000}
A.~Zaffaroni,
\newblock \emph{Introduction to the {AdS}-{CFT} correspondence},
\newblock Classical and Quantum Gravity \textbf{17}(17), 3571 (2000),
\newblock \doi{10.1088/0264-9381/17/17/306}.

\bibitem{Polchinski:2010hw}
J.~Polchinski,
\newblock \emph{{Introduction to Gauge/Gravity Duality}},
\newblock In \emph{{Proceedings, Theoretical Advanced Study Institute in
  Elementary Particle Physics (TASI 2010). String Theory and Its Applications:
  From meV to the Planck Scale: Boulder, Colorado, USA, June 1-25, 2010}}, pp.
  3--46,
\newblock \doi{10.1142/9789814350525_0001} (2010), \eprint{1010.6134}.

\bibitem{Natsuume:2014sfa}
M.~Natsuume,
\newblock \emph{{AdS/CFT Duality User Guide}},
\newblock Lect. Notes Phys. \textbf{903}, pp.1 (2015),
\newblock \doi{10.1007/978-4-431-55441-7},
\newblock \eprint{1409.3575}.

\bibitem{zaanen2015holographic}
J.~Zaanen, Y.~Liu, Y.~Sun and K.~Schalm,
\newblock \emph{Holographic Duality in Condensed Matter Physics},
\newblock Cambridge University Press,
\newblock ISBN 9781107439474 (2015).

\bibitem{Hartnoll:2016apf}
S.~A. Hartnoll, A.~Lucas and S.~Sachdev,
\newblock \emph{{Holographic quantum matter}}  (2016),
\newblock \eprint{1612.07324}.

\bibitem{Hartnoll:2009sz}
S.~A. Hartnoll,
\newblock \emph{{Lectures on holographic methods for condensed matter
  physics}},
\newblock Class. Quant. Grav. \textbf{26}, 224002 (2009),
\newblock \doi{10.1088/0264-9381/26/22/224002},
\newblock \eprint{0903.3246}.

\bibitem{Krikun:2018ufr}
A.~Krikun,
\newblock \emph{{Numerical Solution of the Boundary Value Problems for Partial
  Differential Equations. Crash course for holographer}} (2018),
  \eprint{1801.01483}.

\bibitem{Berti:2009kk}
E.~Berti, V.~Cardoso and A.~O. Starinets,
\newblock \emph{{Quasinormal modes of black holes and black branes}},
\newblock Class. Quant. Grav. \textbf{26}, 163001 (2009),
\newblock \doi{10.1088/0264-9381/26/16/163001},
\newblock \eprint{0905.2975}.

\bibitem{Dias:2015nua}
O.~J.~C. Dias, J.~E. Santos and B.~Way,
\newblock \emph{{Numerical Methods for Finding Stationary Gravitational
  Solutions}},
\newblock Class. Quant. Grav. \textbf{33}(13), 133001 (2016),
\newblock \doi{10.1088/0264-9381/33/13/133001},
\newblock \eprint{1510.02804}.

\bibitem{Jansen:2017oag}
A.~Jansen,
\newblock \emph{{Overdamped modes in Schwarzschild-de Sitter and a Mathematica
  package for the numerical computation of quasinormal modes}},
\newblock Eur. Phys. J. Plus \textbf{132}(12), 546 (2017),
\newblock \doi{10.1140/epjp/i2017-11825-9},
\newblock \eprint{1709.09178}.

\bibitem{Chesler:2013lia}
P.~M. Chesler and L.~G. Yaffe,
\newblock \emph{{Numerical solution of gravitational dynamics in asymptotically
  anti-de Sitter spacetimes}},
\newblock JHEP \textbf{07}, 086 (2014),
\newblock \doi{10.1007/JHEP07(2014)086},
\newblock \eprint{1309.1439}.

\bibitem{Andrade:2017jmt}
T.~Andrade,
\newblock \emph{{Holographic Lattices and Numerical Techniques}} (2017),
  \eprint{1712.00548}.

\bibitem{Zhang:2016coy}
M.~Guo, C.~Niu, Y.~Tian and H.~Zhang,
\newblock \emph{{Applied AdS/CFT with Numerics}},
\newblock PoS \textbf{Modave2015}, 003 (2016),
\newblock \doi{10.22323/1.271.0003},
\newblock \eprint{1601.00257}.

\bibitem{Mathematica10}
{Wolfram Research, Inc.},
\newblock \emph{Mathematica, Version 10.2},
\newblock Champaign, Illinois (2015).

\bibitem{Maldacena:1997re}
J.~M. Maldacena,
\newblock \emph{{The Large N limit of superconformal field theories and
  supergravity}},
\newblock Int. J. Theor. Phys. \textbf{38}, 1113 (1999),
\newblock \doi{10.1023/A:1026654312961, 10.4310/ATMP.1998.v2.n2.a1},
\newblock [Adv. Theor. Math. Phys.2,231(1998)],
\newblock \eprint{hep-th/9711200}.

\bibitem{Witten:1998qj}
E.~Witten,
\newblock \emph{{Anti-de Sitter space and holography}},
\newblock Adv. Theor. Math. Phys. \textbf{2}, 253 (1998),
\newblock \doi{10.4310/ATMP.1998.v2.n2.a2},
\newblock \eprint{hep-th/9802150}.

\bibitem{Giudice:2008bi}
G.~F. Giudice,
\newblock \emph{{Naturally Speaking: The Naturalness Criterion and Physics at
  the LHC}} pp. 155--178 (2008),
\newblock \doi{10.1142/9789812779762_0010},
\newblock \eprint{0801.2562}.

\bibitem{doi:10.1063/1.2735124}
B.~Richter,
\newblock \emph{Is “naturalness” unnatural?},
\newblock AIP Conference Proceedings \textbf{903}(1), 3 (2007),
\newblock \doi{10.1063/1.2735124},
\newblock \eprint{https://aip.scitation.org/doi/pdf/10.1063/1.2735124}.

\bibitem{Palti:2019pca}
E.~Palti,
\newblock \emph{{The Swampland: Introduction and Review}},
\newblock Fortsch. Phys. \textbf{67}(6), 1900037 (2019),
\newblock \doi{10.1002/prop.201900037},
\newblock \eprint{1903.06239}.

\bibitem{fradkin2013field}
E.~Fradkin,
\newblock \emph{Field theories of condensed matter physics},
\newblock Cambridge University Press (2013).

\bibitem{tsvelik2007quantum}
A.~M. Tsvelik,
\newblock \emph{Quantum field theory in condensed matter physics},
\newblock Cambridge university press (2007).

\bibitem{fernandez2000introduction}
F.~M. Fern{\'a}ndez,
\newblock \emph{Introduction to perturbation theory in quantum mechanics},
\newblock CRC press (2000).

\bibitem{scherer2003introduction}
S.~Scherer,
\newblock \emph{Introduction to chiral perturbation theory},
\newblock In \emph{Advances in Nuclear Physics, Volume 27}, pp. 277--538.
  Springer (2003).

\bibitem{kato2012short}
T.~Kato,
\newblock \emph{A short introduction to perturbation theory for linear
  operators},
\newblock Springer Science \& Business Media (2012).

\bibitem{Peskin:1995ev}
M.~E. Peskin and D.~V. Schroeder,
\newblock \emph{{An Introduction to Quantum Field Theory}},
\newblock Westview Press,
\newblock Reading, USA: Addison-Wesley (1995) 842 p (1995).

\bibitem{srednicki2007quantum}
M.~Srednicki,
\newblock \emph{Quantum Field Theory},
\newblock Cambridge University Press,
\newblock ISBN 9781139462761 (2007).

\bibitem{chalupsky2018classical}
J.~Chalupsky,
\newblock \emph{A classical approach to the electron g-factor},
\newblock arXiv preprint arXiv:1806.02274  (2018).

\bibitem{2008PhRvL.100l0801H}
D.~{Hanneke}, S.~{Fogwell} and G.~{Gabrielse},
\newblock \emph{{New Measurement of the Electron Magnetic Moment and the Fine
  Structure Constant}},
\newblock prl \textbf{100}(12), 120801 (2008),
\newblock \doi{10.1103/PhysRevLett.100.120801},
\newblock \eprint{0801.1134}.

\bibitem{Aoyama:2017uqe}
T.~Aoyama, T.~Kinoshita and M.~Nio,
\newblock \emph{{Revised and Improved Value of the QED Tenth-Order Electron
  Anomalous Magnetic Moment}},
\newblock Phys. Rev. \textbf{D97}(3), 036001 (2018),
\newblock \doi{10.1103/PhysRevD.97.036001},
\newblock \eprint{1712.06060}.

\bibitem{PhysRevD.86.010001}
J.~Beringer, J.~F. Arguin, R.~M. Barnett, K.~Copic, O.~Dahl, D.~E. Groom, C.~J.
  Lin, J.~Lys, H.~Murayama, C.~G. Wohl, W.~M. Yao, P.~A. Zyla \emph{et~al.},
\newblock \emph{Review of particle physics},
\newblock Phys. Rev. D \textbf{86}, 010001 (2012),
\newblock \doi{10.1103/PhysRevD.86.010001}.

\bibitem{Teaney:2003kp}
D.~Teaney,
\newblock \emph{{The Effects of viscosity on spectra, elliptic flow, and HBT
  radii}},
\newblock Phys. Rev. \textbf{C68}, 034913 (2003),
\newblock \doi{10.1103/PhysRevC.68.034913},
\newblock \eprint{nucl-th/0301099}.

\bibitem{Arnold:2003zc}
P.~B. Arnold, G.~D. Moore and L.~G. Yaffe,
\newblock \emph{{Transport coefficients in high temperature gauge theories. 2.
  Beyond leading log}},
\newblock JHEP \textbf{05}, 051 (2003),
\newblock \doi{10.1088/1126-6708/2003/05/051},
\newblock \eprint{hep-ph/0302165}.

\bibitem{Huot:2006ys}
S.~C. Huot, S.~Jeon and G.~D. Moore,
\newblock \emph{{Shear viscosity in weakly coupled N = 4 super Yang-Mills
  theory compared to QCD}},
\newblock Phys. Rev. Lett. \textbf{98}, 172303 (2007),
\newblock \doi{10.1103/PhysRevLett.98.172303},
\newblock \eprint{hep-ph/0608062}.

\bibitem{Policastro:2001yc}
G.~Policastro, D.~T. Son and A.~O. Starinets,
\newblock \emph{{The Shear viscosity of strongly coupled N=4 supersymmetric
  Yang-Mills plasma}},
\newblock Phys. Rev. Lett. \textbf{87}, 081601 (2001),
\newblock \doi{10.1103/PhysRevLett.87.081601},
\newblock \eprint{hep-th/0104066}.

\bibitem{Adams_2012}
A.~Adams, L.~D. Carr, T.~Schäfer, P.~Steinberg and J.~E. Thomas,
\newblock \emph{Strongly correlated quantum fluids: ultracold quantum gases,
  quantum chromodynamic plasmas and holographic duality},
\newblock New Journal of Physics \textbf{14}(11), 115009 (2012),
\newblock \doi{10.1088/1367-2630/14/11/115009}.

\bibitem{Bobev:2013cja}
N.~Bobev, H.~Elvang, D.~Z. Freedman and S.~S. Pufu,
\newblock \emph{{Holography for $N = 2^*$ on $S^4$}},
\newblock JHEP \textbf{07}, 001 (2014),
\newblock \doi{10.1007/JHEP07(2014)001},
\newblock \eprint{1311.1508}.

\bibitem{Freedman:2013ryh}
D.~Z. Freedman and S.~S. Pufu,
\newblock \emph{{The holography of $F$-maximization}},
\newblock JHEP \textbf{03}, 135 (2014),
\newblock \doi{10.1007/JHEP03(2014)135},
\newblock \eprint{1302.7310}.

\bibitem{Beisert:2010jr}
N.~Beisert \emph{et~al.},
\newblock \emph{{Review of AdS/CFT Integrability: An Overview}},
\newblock Lett. Math. Phys. \textbf{99}, 3 (2012),
\newblock \doi{10.1007/s11005-011-0529-2},
\newblock \eprint{1012.3982}.

\bibitem{at}
M.~F. Atiyah,
\newblock \emph{{DUALITY IN MATHEMATICS AND PHYSICS}} .

\bibitem{Castellani:2018icz}
E.~Castellani and S.~De~Haro,
\newblock \emph{{Duality, Fundamentality, and Emergence}}  (2018),
\newblock \eprint{1803.09443}.

\bibitem{RevModPhys.52.453}
R.~Savit,
\newblock \emph{Duality in field theory and statistical systems},
\newblock Rev. Mod. Phys. \textbf{52}, 453 (1980),
\newblock \doi{10.1103/RevModPhys.52.453}.

\bibitem{PhysRev.60.252}
H.~A. Kramers and G.~H. Wannier,
\newblock \emph{Statistics of the two-dimensional ferromagnet. part i},
\newblock Phys. Rev. \textbf{60}, 252 (1941),
\newblock \doi{10.1103/PhysRev.60.252}.

\bibitem{Akiyama:2019cqa}
K.~Akiyama \emph{et~al.},
\newblock \emph{{First M87 Event Horizon Telescope Results. I. The Shadow of
  the Supermassive Black Hole}},
\newblock Astrophys. J. \textbf{875}(1), L1 (2019),
\newblock \doi{10.3847/2041-8213/ab0ec7},
\newblock \eprint{1906.11238}.

\bibitem{PhysRevLett.116.061102}
B.~P. Abbott, R.~Abbott, T.~D. Abbott, M.~R. Abernathy, F.~Acernese, K.~Ackley,
  C.~Adams, T.~Adams, P.~Addesso, R.~X. Adhikari, V.~B. Adya, C.~Affeldt
  \emph{et~al.},
\newblock \emph{Observation of gravitational waves from a binary black hole
  merger},
\newblock Phys. Rev. Lett. \textbf{116}, 061102 (2016),
\newblock \doi{10.1103/PhysRevLett.116.061102}.

\bibitem{PhysRevLett.116.241102}
B.~P. Abbott, R.~Abbott, T.~D. Abbott, M.~R. Abernathy, F.~Acernese, K.~Ackley,
  C.~Adams, T.~Adams, P.~Addesso, R.~X. Adhikari, V.~B. Adya, C.~Affeldt
  \emph{et~al.},
\newblock \emph{Properties of the binary black hole merger gw150914},
\newblock Phys. Rev. Lett. \textbf{116}, 241102 (2016),
\newblock \doi{10.1103/PhysRevLett.116.241102}.

\bibitem{Carlip:2014pma}
S.~Carlip,
\newblock \emph{{Black Hole Thermodynamics}},
\newblock Int. J. Mod. Phys. \textbf{D23}, 1430023 (2014),
\newblock \doi{10.1142/S0218271814300237},
\newblock \eprint{1410.1486}.

\bibitem{BekBH}
J.~D. Bekenstein,
\newblock \emph{Black holes and entropy},
\newblock Phys.Rev. D \textbf{7}.

\bibitem{holprinrev}
R.~Bousso,
\newblock \emph{{The Holographic principle}},
\newblock Rev. Mod. Phys. \textbf{74}, 825 (2002),
\newblock \doi{10.1103/RevModPhys.74.825},
\newblock \eprint{hep-th/0203101}.

\bibitem{holprin1}
G.~'t~Hooft,
\newblock \emph{{Dimensional reduction in quantum gravity}},
\newblock In \emph{{Salamfest 1993:0284-296}}, pp. 0284--296 (1993),
  \eprint{gr-qc/9310026}.

\bibitem{holprin2}
L.~Susskind,
\newblock \emph{{The World as a hologram}},
\newblock J. Math. Phys. \textbf{36}, 6377 (1995),
\newblock \doi{10.1063/1.531249},
\newblock \eprint{hep-th/9409089}.

\bibitem{bousso2002holographic}
R.~Bousso,
\newblock \emph{The holographic principle},
\newblock Reviews of Modern Physics \textbf{74}(3), 825 (2002).

\bibitem{Wald:1993nt}
R.~M. Wald,
\newblock \emph{{Black hole entropy is the Noether charge}},
\newblock Phys. Rev. \textbf{D48}(8), R3427 (1993),
\newblock \doi{10.1103/PhysRevD.48.R3427},
\newblock \eprint{gr-qc/9307038}.

\bibitem{Visser:1993nu}
M.~Visser,
\newblock \emph{{Dirty black holes: Entropy as a surface term}},
\newblock Phys. Rev. \textbf{D48}, 5697 (1993),
\newblock \doi{10.1103/PhysRevD.48.5697},
\newblock \eprint{hep-th/9307194}.

\bibitem{Brustein:2007jj}
R.~Brustein, D.~Gorbonos and M.~Hadad,
\newblock \emph{{Wald's entropy is equal to a quarter of the horizon area in
  units of the effective gravitational coupling}},
\newblock Phys. Rev. \textbf{D79}, 044025 (2009),
\newblock \doi{10.1103/PhysRevD.79.044025},
\newblock \eprint{0712.3206}.

\bibitem{Horndeski1974}
G.~W. Horndeski,
\newblock \emph{Second-order scalar-tensor field equations in a
  four-dimensional space},
\newblock International Journal of Theoretical Physics \textbf{10}(6), 363
  (1974),
\newblock \doi{10.1007/BF01807638}.

\bibitem{Deffayet:2013lga}
C.~Deffayet and D.~A. Steer,
\newblock \emph{{A formal introduction to Horndeski and Galileon theories and
  their generalizations}},
\newblock Class. Quant. Grav. \textbf{30}, 214006 (2013),
\newblock \doi{10.1088/0264-9381/30/21/214006},
\newblock \eprint{1307.2450}.

\bibitem{Baggioli:2017ojd}
M.~Baggioli and W.-J. Li,
\newblock \emph{{Diffusivities bounds and chaos in holographic Horndeski
  theories}},
\newblock JHEP \textbf{07}, 055 (2017),
\newblock \doi{10.1007/JHEP07(2017)055},
\newblock \eprint{1705.01766}.

\bibitem{Kats:2007mq}
Y.~Kats and P.~Petrov,
\newblock \emph{{Effect of curvature squared corrections in AdS on the
  viscosity of the dual gauge theory}},
\newblock JHEP \textbf{01}, 044 (2009),
\newblock \doi{10.1088/1126-6708/2009/01/044},
\newblock \eprint{0712.0743}.

\bibitem{doi:10.1063/1.1665613}
D.~Lovelock,
\newblock \emph{The einstein tensor and its generalizations},
\newblock Journal of Mathematical Physics \textbf{12}(3), 498 (1971),
\newblock \doi{10.1063/1.1665613},
\newblock \eprint{https://doi.org/10.1063/1.1665613}.

\bibitem{RevModPhys.47.773}
K.~G. Wilson,
\newblock \emph{The renormalization group: Critical phenomena and the kondo
  problem},
\newblock Rev. Mod. Phys. \textbf{47}, 773 (1975),
\newblock \doi{10.1103/RevModPhys.47.773}.

\bibitem{adscftMcGreevy}
J.~McGreevy,
\newblock \emph{{Holographic duality with a view toward many-body physics}},
\newblock Adv. High Energy Phys. \textbf{2010}, 723105 (2010),
\newblock \doi{10.1155/2010/723105},
\newblock \eprint{0909.0518}.

\bibitem{Lee:2013dln}
S.-S. Lee,
\newblock \emph{{Quantum Renormalization Group and Holography}},
\newblock JHEP \textbf{01}, 076 (2014),
\newblock \doi{10.1007/JHEP01(2014)076},
\newblock \eprint{1305.3908}.

\bibitem{Lee:2012xba}
S.-S. Lee,
\newblock \emph{{Background independent holographic description : From matrix
  field theory to quantum gravity}},
\newblock JHEP \textbf{10}, 160 (2012),
\newblock \doi{10.1007/JHEP10(2012)160},
\newblock \eprint{1204.1780}.

\bibitem{Lee:2010ub}
S.-S. Lee,
\newblock \emph{{Holographic description of large N gauge theory}},
\newblock Nucl. Phys. \textbf{B851}, 143 (2011),
\newblock \doi{10.1016/j.nuclphysb.2011.05.011},
\newblock \eprint{1011.1474}.

\bibitem{Lee:2009ij}
S.-S. Lee,
\newblock \emph{{Holographic description of quantum field theory}},
\newblock Nucl. Phys. \textbf{B832}, 567 (2010),
\newblock \doi{10.1016/j.nuclphysb.2010.02.022},
\newblock \eprint{0912.5223}.

\bibitem{Mukhopadhyay:2017uik}
A.~Mukhopadhyay,
\newblock \emph{{Emergence of Gravity and RG Flow}},
\newblock Fundam. Theor. Phys. \textbf{187}, 283 (2017),
\newblock \doi{10.1007/978-3-319-51700-1_17}.

\bibitem{Mukhopadhyay:2016fre}
A.~Mukhopadhyay,
\newblock \emph{{Understanding the holographic principle via RG flow}},
\newblock Int. J. Mod. Phys. \textbf{A31}(34), 1630059 (2016),
\newblock \doi{10.1142/S0217751X16300593},
\newblock \eprint{1612.00141}.

\bibitem{Behr:2015aat}
N.~Behr and A.~Mukhopadhyay,
\newblock \emph{{Holography as a highly efficient renormalization group flow.
  II. An explicit construction}},
\newblock Phys. Rev. \textbf{D94}(2), 026002 (2016),
\newblock \doi{10.1103/PhysRevD.94.026002},
\newblock \eprint{1512.09055}.

\bibitem{Behr:2015yna}
N.~Behr, S.~Kuperstein and A.~Mukhopadhyay,
\newblock \emph{{Holography as a highly efficient renormalization group flow.
  I. Rephrasing gravity}},
\newblock Phys. Rev. \textbf{D94}(2), 026001 (2016),
\newblock \doi{10.1103/PhysRevD.94.026001},
\newblock \eprint{1502.06619}.

\bibitem{Baggioli:2016rdj}
M.~Baggioli,
\newblock \emph{{Gravity, holography and applications to condensed matter}},
\newblock Ph.D. thesis, Barcelona U. (2016), \eprint{1610.02681}.

\bibitem{largeNQFT}
M.~Moshe and J.~Zinn-Justin,
\newblock \emph{{Quantum field theory in the large N limit: A Review}},
\newblock Phys. Rept. \textbf{385}, 69 (2003),
\newblock \doi{10.1016/S0370-1573(03)00263-1},
\newblock \eprint{hep-th/0306133}.

\bibitem{thooftN}
G.~Hooft,
\newblock \emph{A planar diagram theory for strong interactions},
\newblock Nuclear Physics B \textbf{72}.

\bibitem{Lucini:2012gg}
B.~Lucini and M.~Panero,
\newblock \emph{{SU(N) gauge theories at large N}},
\newblock Phys. Rept. \textbf{526}, 93 (2013),
\newblock \doi{10.1016/j.physrep.2013.01.001},
\newblock \eprint{1210.4997}.

\bibitem{adscftZaffaroni}
A.Zaffaroni,
\newblock \emph{Introduction to the ads-cft correspondence},
\newblock Class.Quant.Grav. \textbf{17}.

\bibitem{polchinski2001string}
J.~Polchinski,
\newblock \emph{String Theory},
\newblock String Theory 2 Volume Hardback Set. Cambridge University Press,
\newblock ISBN 9780521633031 (2001).

\bibitem{zwiebach2004first}
B.~Zwiebach and C.~U. Press,
\newblock \emph{A First Course in String Theory},
\newblock A First Course in String Theory. Cambridge University Press,
\newblock ISBN 9780521831437 (2004).

\bibitem{Hartnoll:2008vx}
S.~A. Hartnoll, C.~P. Herzog and G.~T. Horowitz,
\newblock \emph{{Building a Holographic Superconductor}},
\newblock Phys. Rev. Lett. \textbf{101}, 031601 (2008),
\newblock \doi{10.1103/PhysRevLett.101.031601},
\newblock \eprint{0803.3295}.

\bibitem{Hartnoll:2008kx}
S.~A. Hartnoll, C.~P. Herzog and G.~T. Horowitz,
\newblock \emph{{Holographic Superconductors}},
\newblock JHEP \textbf{12}, 015 (2008),
\newblock \doi{10.1088/1126-6708/2008/12/015},
\newblock \eprint{0810.1563}.

\bibitem{Domenech:2010nf}
O.~Domenech, M.~Montull, A.~Pomarol, A.~Salvio and P.~J. Silva,
\newblock \emph{{Emergent Gauge Fields in Holographic Superconductors}},
\newblock JHEP \textbf{08}, 033 (2010),
\newblock \doi{10.1007/JHEP08(2010)033},
\newblock \eprint{1005.1776}.

\bibitem{PhysRevLett.17.1133}
N.~D. Mermin and H.~Wagner,
\newblock \emph{Absence of ferromagnetism or antiferromagnetism in one- or
  two-dimensional isotropic heisenberg models},
\newblock Phys. Rev. Lett. \textbf{17}, 1133 (1966),
\newblock \doi{10.1103/PhysRevLett.17.1133}.

\bibitem{Coleman1973}
S.~Coleman,
\newblock \emph{There are no goldstone bosons in two dimensions},
\newblock Communications in Mathematical Physics \textbf{31}(4), 259 (1973),
\newblock \doi{10.1007/BF01646487}.

\bibitem{Merkl1994}
F.~Merkl and H.~Wagner,
\newblock \emph{Recurrent random walks and the absence of continuous symmetry
  breaking on graphs},
\newblock Journal of Statistical Physics \textbf{75}(1), 153 (1994),
\newblock \doi{10.1007/BF02186284}.

\bibitem{PhysRevD.11.1701}
S.-k. Ma and R.~Rajaraman,
\newblock \emph{Comments on the absence of spontaneous symmetry breaking in low
  dimensions},
\newblock Phys. Rev. D \textbf{11}, 1701 (1975),
\newblock \doi{10.1103/PhysRevD.11.1701}.

\bibitem{Anninos:2010sq}
D.~Anninos, S.~A. Hartnoll and N.~Iqbal,
\newblock \emph{{Holography and the Coleman-Mermin-Wagner theorem}},
\newblock Phys. Rev. \textbf{D82}, 066008 (2010),
\newblock \doi{10.1103/PhysRevD.82.066008},
\newblock \eprint{1005.1973}.

\bibitem{Grozdanov:2015qia}
S.~Grozdanov, A.~Lucas, S.~Sachdev and K.~Schalm,
\newblock \emph{{Absence of disorder-driven metal-insulator transitions in
  simple holographic models}},
\newblock Phys. Rev. Lett. \textbf{115}(22), 221601 (2015),
\newblock \doi{10.1103/PhysRevLett.115.221601},
\newblock \eprint{1507.00003}.

\bibitem{Sarkar:2010zza}
S.~Sarkar, H.~Satz and B.~Sinha,
\newblock \emph{{The physics of the quark-gluon plasma}},
\newblock Lect. Notes Phys. \textbf{785}, pp.1 (2010),
\newblock \doi{10.1007/978-3-642-02286-9}.

\bibitem{Gupta:1997nd}
R.~Gupta,
\newblock \emph{{Introduction to lattice QCD: Course}},
\newblock In \emph{{Probing the standard model of particle interactions.
  Proceedings, Summer School in Theoretical Physics, NATO Advanced Study
  Institute, 68th session, Les Houches, France, July 28-September 5, 1997. Pt.
  1, 2}}, pp. 83--219 (1997), \eprint{hep-lat/9807028}.

\bibitem{Csaki:2008dt}
C.~Csaki, M.~Reece and J.~Terning,
\newblock \emph{{The AdS/QCD Correspondence: Still Undelivered}},
\newblock JHEP \textbf{05}, 067 (2009),
\newblock \doi{10.1088/1126-6708/2009/05/067},
\newblock \eprint{0811.3001}.

\bibitem{bogoliuubov1963theory}
N.~Bogoliubov,
\newblock \emph{Theory of Superconductivity},
\newblock No. v. 4 in International science review series. Gordon and Breach,
\newblock ISBN 9780677000800 (1963).

\bibitem{tinkham2004introduction}
M.~Tinkham,
\newblock \emph{Introduction to Superconductivity},
\newblock Dover Books on Physics Series. Dover Publications,
\newblock ISBN 9780486134727 (2004).

\bibitem{1986ZPhyB..64..189B}
J.~G. {Bednorz} and K.~A. {M{\"u}ller},
\newblock \emph{{Possible high T$_{c}$ superconductivity in the Ba-La-Cu-O
  system}},
\newblock Zeitschrift fur Physik B Condensed Matter \textbf{64}, 189 (1986),
\newblock \doi{10.1007/BF01303701}.

\bibitem{Leggett2006}
A.~J. Leggett,
\newblock \emph{What do we know about high tc?},
\newblock Nature Physics \textbf{2}(3), 134 (2006),
\newblock \doi{10.1038/nphys254}.

\bibitem{Drozdov2019}
A.~P. Drozdov, P.~P. Kong, V.~S. Minkov, S.~P. Besedin, M.~A. Kuzovnikov,
  S.~Mozaffari, L.~Balicas, F.~F. Balakirev, D.~E. Graf, V.~B. Prakapenka,
  E.~Greenberg, D.~A. Knyazev \emph{et~al.},
\newblock \emph{Superconductivity at 250 k in lanthanum hydride under high
  pressures},
\newblock Nature \textbf{569}(7757), 528 (2019),
\newblock \doi{10.1038/s41586-019-1201-8}.

\bibitem{song2017phonon}
Q.~Song, T.~Yu, X.~Lou, B.~Xie, H.~C. Xu, C.~Wen, Q.~Yao, S.~Zhang, X.~Zhu,
  J.~Guo \emph{et~al.},
\newblock \emph{Phonon-enhanced superconductivity at the fese/srtio3
  interface},
\newblock arXiv preprint arXiv:1710.07057  (2017).

\bibitem{Cooper603}
R.~A. Cooper, Y.~Wang, B.~Vignolle, O.~J. Lipscombe, S.~M. Hayden, Y.~Tanabe,
  T.~Adachi, Y.~Koike, M.~Nohara, H.~Takagi, C.~Proust and N.~E. Hussey,
\newblock \emph{Anomalous criticality in the electrical resistivity of
  la2{\textendash}xsrxcuo4},
\newblock Science \textbf{323}(5914), 603 (2009),
\newblock \doi{10.1126/science.1165015},
\newblock
  \eprint{https://science.sciencemag.org/content/323/5914/603.full.pdf}.

\bibitem{PhysRevLett.74.3253}
V.~J. Emery and S.~A. Kivelson,
\newblock \emph{Superconductivity in bad metals},
\newblock Phys. Rev. Lett. \textbf{74}, 3253 (1995),
\newblock \doi{10.1103/PhysRevLett.74.3253}.

\bibitem{hirsch2001electron}
J.~Hirsch and F.~Marsiglio,
\newblock \emph{Electron-phonon or hole superconductivity in mgb 2},
\newblock Physical Review B \textbf{64}(14), 144523 (2001).

\bibitem{Kovtun:2012rj}
P.~Kovtun,
\newblock \emph{{Lectures on hydrodynamic fluctuations in relativistic
  theories}},
\newblock J. Phys. \textbf{A45}, 473001 (2012),
\newblock \doi{10.1088/1751-8113/45/47/473001},
\newblock \eprint{1205.5040}.

\bibitem{landau1986theory}
L.~Landau, E.~Lifshitz, A.~Kosevich, J.~Sykes, L.~Pitaevskii and W.~Reid,
\newblock \emph{Theory of Elasticity},
\newblock Course of theoretical physics. Elsevier Science,
\newblock ISBN 9780750626330 (1986).

\bibitem{chaikin2000principles}
P.~Chaikin and T.~Lubensky,
\newblock \emph{Principles of Condensed Matter Physics},
\newblock Cambridge University Press,
\newblock ISBN 9780521794503 (2000).

\bibitem{Policastro:2002se}
G.~Policastro, D.~T. Son and A.~O. Starinets,
\newblock \emph{{From AdS / CFT correspondence to hydrodynamics}},
\newblock JHEP \textbf{09}, 043 (2002),
\newblock \doi{10.1088/1126-6708/2002/09/043},
\newblock \eprint{hep-th/0205052}.

\bibitem{Policastro:2002tn}
G.~Policastro, D.~T. Son and A.~O. Starinets,
\newblock \emph{{From AdS / CFT correspondence to hydrodynamics. 2. Sound
  waves}},
\newblock JHEP \textbf{12}, 054 (2002),
\newblock \doi{10.1088/1126-6708/2002/12/054},
\newblock \eprint{hep-th/0210220}.

\bibitem{Grozdanov:2013dba}
S.~Grozdanov and J.~Polonyi,
\newblock \emph{{Viscosity and dissipative hydrodynamics from effective field
  theory}},
\newblock Phys. Rev. \textbf{D91}(10), 105031 (2015),
\newblock \doi{10.1103/PhysRevD.91.105031},
\newblock \eprint{1305.3670}.

\bibitem{Jensen:2018hse}
K.~Jensen, R.~Marjieh, N.~Pinzani-Fokeeva and A.~Yarom,
\newblock \emph{{A panoply of Schwinger-Keldysh transport}},
\newblock SciPost Phys. \textbf{5}(5), 053 (2018),
\newblock \doi{10.21468/SciPostPhys.5.5.053},
\newblock \eprint{1804.04654}.

\bibitem{Jensen:2017kzi}
K.~Jensen, N.~Pinzani-Fokeeva and A.~Yarom,
\newblock \emph{{Dissipative hydrodynamics in superspace}},
\newblock JHEP \textbf{09}, 127 (2018),
\newblock \doi{10.1007/JHEP09(2018)127},
\newblock \eprint{1701.07436}.

\bibitem{Glorioso:2018wxw}
H.~Liu and P.~Glorioso,
\newblock \emph{{Lectures on non-equilibrium effective field theories and
  fluctuating hydrodynamics}},
\newblock PoS \textbf{TASI2017}, 008 (2018),
\newblock \doi{10.22323/1.305.0008},
\newblock \eprint{1805.09331}.

\bibitem{Haehl:2017zac}
F.~M. Haehl, R.~Loganayagam and M.~Rangamani,
\newblock \emph{{Two roads to hydrodynamic effective actions: a comparison}}
  (2017),
\newblock \eprint{1701.07896}.

\bibitem{Crossley:2015evo}
M.~Crossley, P.~Glorioso and H.~Liu,
\newblock \emph{{Effective field theory of dissipative fluids}},
\newblock JHEP \textbf{09}, 095 (2017),
\newblock \doi{10.1007/JHEP09(2017)095},
\newblock \eprint{1511.03646}.

\bibitem{Haehl:2018lcu}
F.~M. Haehl, R.~Loganayagam and M.~Rangamani,
\newblock \emph{{Effective Action for Relativistic Hydrodynamics: Fluctuations,
  Dissipation, and Entropy Inflow}},
\newblock JHEP \textbf{10}, 194 (2018),
\newblock \doi{10.1007/JHEP10(2018)194},
\newblock \eprint{1803.11155}.

\bibitem{Haehl:2015foa}
F.~M. Haehl, R.~Loganayagam and M.~Rangamani,
\newblock \emph{{The Fluid Manifesto: Emergent symmetries, hydrodynamics, and
  black holes}},
\newblock JHEP \textbf{01}, 184 (2016),
\newblock \doi{10.1007/JHEP01(2016)184},
\newblock \eprint{1510.02494}.

\bibitem{Baggioli:2019abx}
M.~Baggioli and S.~Grieninger,
\newblock \emph{{Zoology of Solid \& Fluid Holography : Goldstone Modes and
  Phase Relaxation}}  (2019),
\newblock \eprint{1905.09488}.

\bibitem{Leutwyler:1996er}
H.~Leutwyler,
\newblock \emph{{Phonons as goldstone bosons}},
\newblock Helv. Phys. Acta \textbf{70}, 275 (1997),
\newblock \eprint{hep-ph/9609466}.

\bibitem{Endlich:2012vt}
S.~Endlich, A.~Nicolis, R.~A. Porto and J.~Wang,
\newblock \emph{{Dissipation in the effective field theory for hydrodynamics:
  First order effects}},
\newblock Phys. Rev. \textbf{D88}, 105001 (2013),
\newblock \doi{10.1103/PhysRevD.88.105001},
\newblock \eprint{1211.6461}.

\bibitem{bender2007making}
C.~M. Bender,
\newblock \emph{Making sense of non-hermitian hamiltonians},
\newblock Reports on Progress in Physics \textbf{70}(6), 947 (2007).

\bibitem{1986bhmp.book.....T}
K.~S. {Thorne}, R.~H. {Price} and D.~A. {MacDonald},
\newblock \emph{{Black holes: The membrane paradigm}} (1986).

\bibitem{PhysRevD.18.3598}
T.~Damour,
\newblock \emph{Black-hole eddy currents},
\newblock Phys. Rev. D \textbf{18}, 3598 (1978),
\newblock \doi{10.1103/PhysRevD.18.3598}.

\bibitem{Cohen:2019wxr}
T.~Cohen,
\newblock \emph{{As Scales Become Separated: Lectures on Effective Field
  Theory}}  (2019),
\newblock \eprint{1903.03622}.

\bibitem{Hartnoll2014}
S.~A. Hartnoll,
\newblock \emph{Theory of universal incoherent metallic transport},
\newblock Nature Physics \textbf{11}, 54 EP  (2014),
\newblock Article.

\bibitem{hussey2004universality}
N.~Hussey, K.~Takenaka and H.~Takagi,
\newblock \emph{Universality of the mott--ioffe--regel limit in metals},
\newblock Philosophical Magazine \textbf{84}(27), 2847 (2004).

\bibitem{allen2002quasi}
J.~Allen,
\newblock \emph{Quasi-particles and their absence in photoemission
  spectroscopy},
\newblock Solid state communications \textbf{123}(11), 469 (2002).

\bibitem{harris2012introduction}
S.~Harris,
\newblock \emph{An Introduction to the Theory of the Boltzmann Equation},
\newblock Dover Books on Physics. Dover Publications,
\newblock ISBN 9780486143828 (2012).

\bibitem{Chemissany:2014xsa}
W.~Chemissany and I.~Papadimitriou,
\newblock \emph{{Lifshitz holography: The whole shebang}},
\newblock JHEP \textbf{01}, 052 (2015),
\newblock \doi{10.1007/JHEP01(2015)052},
\newblock \eprint{1408.0795}.

\bibitem{blumenhagen2009introduction}
R.~Blumenhagen and E.~Plauschinn,
\newblock \emph{Introduction to Conformal Field Theory: With Applications to
  String Theory},
\newblock Lecture Notes in Physics. Springer Berlin Heidelberg,
\newblock ISBN 9783642004490 (2009).

\bibitem{gaberdiel2000introduction}
M.~R. Gaberdiel,
\newblock \emph{An introduction to conformal field theory},
\newblock Reports on Progress in Physics \textbf{63}(4), 607 (2000).

\bibitem{Witten1}
E.~Witten,
\newblock \emph{{Anti-de Sitter space and holography}},
\newblock Adv. Theor. Math. Phys. \textbf{2}, 253 (1998),
\newblock \eprint{hep-th/9802150}.

\bibitem{GPKW1}
S.~S. Gubser, I.~R. Klebanov and A.~M. Polyakov,
\newblock \emph{{Gauge theory correlators from noncritical string theory}},
\newblock Phys. Lett. \textbf{B428}, 105 (1998),
\newblock \doi{10.1016/S0370-2693(98)00377-3},
\newblock \eprint{hep-th/9802109}.

\bibitem{Marolf:2006nd}
D.~Marolf and S.~F. Ross,
\newblock \emph{{Boundary Conditions and New Dualities: Vector Fields in
  AdS/CFT}},
\newblock JHEP \textbf{11}, 085 (2006),
\newblock \doi{10.1088/1126-6708/2006/11/085},
\newblock \eprint{hep-th/0606113}.

\bibitem{Witten:2001ua}
E.~Witten,
\newblock \emph{{Multitrace operators, boundary conditions, and AdS / CFT
  correspondence}}  (2001),
\newblock \eprint{hep-th/0112258}.

\bibitem{Witten:2003ya}
E.~Witten,
\newblock \emph{{SL(2,Z) action on three-dimensional conformal field theories
  with Abelian symmetry}} pp. 1173--1200 (2003),
\newblock \eprint{hep-th/0307041}.

\bibitem{Yee:2004ju}
H.-U. Yee,
\newblock \emph{{A Note on AdS / CFT dual of SL(2,Z) action on 3-D conformal
  field theories with U(1) symmetry}},
\newblock Phys. Lett. \textbf{B598}, 139 (2004),
\newblock \doi{10.1016/j.physletb.2004.05.082},
\newblock \eprint{hep-th/0402115}.

\bibitem{Andrade:2013wsa}
T.~Andrade and S.~F. Ross,
\newblock \emph{{Boundary conditions for metric fluctuations in Lifshitz}},
\newblock Class. Quant. Grav. \textbf{30}, 195017 (2013),
\newblock \doi{10.1088/0264-9381/30/19/195017},
\newblock \eprint{1305.3539}.

\bibitem{Jokela:2013hta}
N.~Jokela, G.~Lifschytz and M.~Lippert,
\newblock \emph{{Holographic anyonic superfluidity}},
\newblock JHEP \textbf{10}, 014 (2013),
\newblock \doi{10.1007/JHEP10(2013)014},
\newblock \eprint{1307.6336}.

\bibitem{Aronsson:2017dgf}
U.~Gran, M.~Tornsö and T.~Zingg,
\newblock \emph{{Holographic Plasmons}},
\newblock JHEP \textbf{11}, 176 (2018),
\newblock \doi{10.1007/JHEP11(2018)176},
\newblock \eprint{1712.05672}.

\bibitem{Baggioli:2019aqf}
M.~Baggioli, U.~Gran, A.~J. Alba, M.~Tornsö and T.~Zingg,
\newblock \emph{{Holographic Plasmon Relaxation with and without Broken
  Translations}}  (2019),
\newblock \eprint{1905.00804}.

\bibitem{Armas:2019sbe}
J.~Armas and A.~Jain,
\newblock \emph{{Viscoelastic hydrodynamics and holography}}  (2019),
\newblock \eprint{1908.01175}.

\bibitem{Skenderis1}
K.~Skenderis,
\newblock \emph{{Lecture notes on holographic renormalization}},
\newblock Class. Quant. Grav. \textbf{19}, 5849 (2002),
\newblock \doi{10.1088/0264-9381/19/22/306},
\newblock \eprint{hep-th/0209067}.

\bibitem{Linear1}
T.~S.~V. Bonch-Bruevich V.~L.,
\newblock \emph{The Green Function Method in Statistical Mechanics},
\newblock North Holland Publishing Co. (1962).

\bibitem{BFpaper}
P.~Breitenlohner and D.~Freedman,
\newblock \emph{“stability in gauged extended supergravity},
\newblock Ann. Phys. \textbf{144}, 249.

\bibitem{wald1}
Q.~F.~T. in~Curved~Spacetime and B.~H. Thermodynamics,
\newblock \emph{R.Wald},
\newblock University of Chicago Press (1994).

\bibitem{unbounds}
S.~Minwalla,
\newblock \emph{{Restrictions imposed by superconformal invariance on quantum
  field theories}},
\newblock Adv. Theor. Math. Phys. \textbf{2}, 781 (1998),
\newblock \eprint{hep-th/9712074}.

\bibitem{landau2013fluid}
L.~Landau and E.~Lifshitz,
\newblock \emph{Fluid Mechanics},
\newblock v. 6. Elsevier Science,
\newblock ISBN 9781483140506 (2013).

\bibitem{PhysRevA.6.2401}
P.~C. Martin, O.~Parodi and P.~S. Pershan,
\newblock \emph{Unified hydrodynamic theory for crystals, liquid crystals, and
  normal fluids},
\newblock Phys. Rev. A \textbf{6}, 2401 (1972),
\newblock \doi{10.1103/PhysRevA.6.2401}.

\bibitem{forster1975hydrodynamic}
D.~Forster,
\newblock \emph{Hydrodynamic fluctuations, broken symmetry, and correlation
  functions},
\newblock Frontiers in Physics : a lecture note and reprint series. W. A.
  Benjamin, Advanced Book Program (1975).

\bibitem{boon1991molecular}
J.~Boon and S.~Yip,
\newblock \emph{Molecular Hydrodynamics},
\newblock Dover books on physics. Dover Publications,
\newblock ISBN 9780486669496 (1991).

\bibitem{Grozdanov:2018fic}
S.~Grozdanov, A.~Lucas and N.~Poovuttikul,
\newblock \emph{{Holography and hydrodynamics with weakly broken symmetries}},
\newblock Phys. Rev. \textbf{D99}(8), 086012 (2019),
\newblock \doi{10.1103/PhysRevD.99.086012},
\newblock \eprint{1810.10016}.

\bibitem{soon}
M.~Baggioli, V.~Cancer~Castillo and O.~Pujolas,
\newblock \emph{Scale invariant solids},
\newblock To Appear  (2019).

\bibitem{PhysRev.85.631}
F.~J. Dyson,
\newblock \emph{Divergence of perturbation theory in quantum electrodynamics},
\newblock Phys. Rev. \textbf{85}, 631 (1952),
\newblock \doi{10.1103/PhysRev.85.631}.

\bibitem{Withers:2018srf}
B.~Withers,
\newblock \emph{{Short-lived modes from hydrodynamic dispersion relations}},
\newblock JHEP \textbf{06}, 059 (2018),
\newblock \doi{10.1007/JHEP06(2018)059},
\newblock \eprint{1803.08058}.

\bibitem{Grozdanov:2019kge}
S.~Grozdanov, P.~K. Kovtun, A.~O. Starinets and P.~Tadić,
\newblock \emph{{On the convergence of the gradient expansion in
  hydrodynamics}},
\newblock Phys. Rev. Lett. \textbf{122}(25), 251601 (2019),
\newblock \doi{10.1103/PhysRevLett.122.251601},
\newblock \eprint{1904.01018}.

\bibitem{Grozdanov:2019uhi}
S.~Grozdanov, P.~K. Kovtun, A.~O. Starinets and P.~Tadić,
\newblock \emph{{The complex life of hydrodynamic modes}}  (2019),
\newblock \eprint{1904.12862}.

\bibitem{Heller:2016rtz}
M.~P. Heller, A.~Kurkela, M.~Spaliński and V.~Svensson,
\newblock \emph{{Hydrodynamization in kinetic theory: Transient modes and the
  gradient expansion}},
\newblock Phys. Rev. \textbf{D97}(9), 091503 (2018),
\newblock \doi{10.1103/PhysRevD.97.091503},
\newblock \eprint{1609.04803}.

\bibitem{Baggioli:2018bfa}
M.~Baggioli and A.~Buchel,
\newblock \emph{{Holographic Viscoelastic Hydrodynamics}},
\newblock JHEP \textbf{03}, 146 (2019),
\newblock \doi{10.1007/JHEP03(2019)146},
\newblock \eprint{1805.06756}.

\bibitem{Buchel:2016cbj}
A.~Buchel, M.~P. Heller and J.~Noronha,
\newblock \emph{{Entropy Production, Hydrodynamics, and Resurgence in the
  Primordial Quark-Gluon Plasma from Holography}},
\newblock Phys. Rev. \textbf{D94}(10), 106011 (2016),
\newblock \doi{10.1103/PhysRevD.94.106011},
\newblock \eprint{1603.05344}.

\bibitem{Aniceto:2018uik}
I.~Aniceto, B.~Meiring, J.~Jankowski and M.~Spaliński,
\newblock \emph{{The large proper-time expansion of Yang-Mills plasma as a
  resurgent transseries}},
\newblock JHEP \textbf{02}, 073 (2019),
\newblock \doi{10.1007/JHEP02(2019)073},
\newblock \eprint{1810.07130}.

\bibitem{Aniceto:2015mto}
I.~Aniceto and M.~Spaliński,
\newblock \emph{{Resurgence in Extended Hydrodynamics}},
\newblock Phys. Rev. \textbf{D93}(8), 085008 (2016),
\newblock \doi{10.1103/PhysRevD.93.085008},
\newblock \eprint{1511.06358}.

\bibitem{Heller:2015dha}
M.~P. Heller and M.~Spalinski,
\newblock \emph{{Hydrodynamics Beyond the Gradient Expansion: Resurgence and
  Resummation}},
\newblock Phys. Rev. Lett. \textbf{115}(7), 072501 (2015),
\newblock \doi{10.1103/PhysRevLett.115.072501},
\newblock \eprint{1503.07514}.

\bibitem{Dubovsky:2011sj}
S.~Dubovsky, L.~Hui, A.~Nicolis and D.~T. Son,
\newblock \emph{{Effective field theory for hydrodynamics: thermodynamics, and
  the derivative expansion}},
\newblock Phys. Rev. \textbf{D85}, 085029 (2012),
\newblock \doi{10.1103/PhysRevD.85.085029},
\newblock \eprint{1107.0731}.

\bibitem{wald2010general}
R.~Wald,
\newblock \emph{General Relativity},
\newblock University of Chicago Press,
\newblock ISBN 9780226870373 (2010).

\bibitem{weinberg1972gravitation}
S.~Weinberg,
\newblock \emph{Gravitation and cosmology: principles and applications of the
  general theory of relativity},
\newblock Wiley,
\newblock ISBN 9780471925675 (1972).

\bibitem{Zaanen:2018edk}
J.~Zaanen,
\newblock \emph{{Planckian dissipation, minimal viscosity and the transport in
  cuprate strange metals}},
\newblock SciPost Phys. \textbf{6}(5), 061 (2019),
\newblock \doi{10.21468/SciPostPhys.6.5.061},
\newblock \eprint{1807.10951}.

\bibitem{Cremonini:2011iq}
S.~Cremonini,
\newblock \emph{{The Shear Viscosity to Entropy Ratio: A Status Report}},
\newblock Mod. Phys. Lett. \textbf{B25}, 1867 (2011),
\newblock \doi{10.1142/S0217984911027315},
\newblock \eprint{1108.0677}.

\bibitem{Cremonini:2012ny}
S.~Cremonini, U.~Gursoy and P.~Szepietowski,
\newblock \emph{{On the Temperature Dependence of the Shear Viscosity and
  Holography}},
\newblock JHEP \textbf{08}, 167 (2012),
\newblock \doi{10.1007/JHEP08(2012)167},
\newblock \eprint{1206.3581}.

\bibitem{Son:2002sd}
D.~T. Son and A.~O. Starinets,
\newblock \emph{{Minkowski space correlators in AdS / CFT correspondence:
  Recipe and applications}},
\newblock JHEP \textbf{09}, 042 (2002),
\newblock \doi{10.1088/1126-6708/2002/09/042},
\newblock \eprint{hep-th/0205051}.

\bibitem{Iqbal:2008by}
N.~Iqbal and H.~Liu,
\newblock \emph{{Universality of the hydrodynamic limit in AdS/CFT and the
  membrane paradigm}},
\newblock Phys. Rev. \textbf{D79}, 025023 (2009),
\newblock \doi{10.1103/PhysRevD.79.025023},
\newblock \eprint{0809.3808}.

\bibitem{Kovtun:2004de}
P.~Kovtun, D.~T. Son and A.~O. Starinets,
\newblock \emph{{Viscosity in strongly interacting quantum field theories from
  black hole physics}},
\newblock Phys. Rev. Lett. \textbf{94}, 111601 (2005),
\newblock \doi{10.1103/PhysRevLett.94.111601},
\newblock \eprint{hep-th/0405231}.

\bibitem{Noirez_2012}
L.~Noirez and P.~Baroni,
\newblock \emph{Identification of a low-frequency elastic behaviour in liquid
  water},
\newblock Journal of Physics: Condensed Matter \textbf{24}(37), 372101 (2012),
\newblock \doi{10.1088/0953-8984/24/37/372101}.

\bibitem{yang2017emergence}
C.~Yang, M.~Dove, V.~Brazhkin and K.~Trachenko,
\newblock \emph{Emergence and evolution of the k gap in spectra of liquid and
  supercritical states},
\newblock Physical review letters \textbf{118}(21), 215502 (2017).

\bibitem{trachenko2015collective}
K.~Trachenko and V.~Brazhkin,
\newblock \emph{Collective modes and thermodynamics of the liquid state},
\newblock Reports on Progress in Physics \textbf{79}(1), 016502 (2015).

\bibitem{Baggioli:2019jcm}
M.~Baggioli, M.~Vasin, V.~V. Brazhkin and K.~Trachenko,
\newblock \emph{{Gapped momentum states}}  (2019),
\newblock \eprint{1904.01419}.

\bibitem{Baggioli:2018nnp}
M.~Baggioli and K.~Trachenko,
\newblock \emph{{Maxwell interpolation and close similarities between liquids
  and holographic models}}  (2018),
\newblock \eprint{1808.05391}.

\bibitem{Baggioli:2018vfc}
M.~Baggioli and K.~Trachenko,
\newblock \emph{{Low frequency propagating shear waves in holographic
  liquids}},
\newblock JHEP \textbf{03}, 093 (2019),
\newblock \doi{10.1007/JHEP03(2019)093},
\newblock \eprint{1807.10530}.

\bibitem{Brigante:2007nu}
M.~Brigante, H.~Liu, R.~C. Myers, S.~Shenker and S.~Yaida,
\newblock \emph{{Viscosity Bound Violation in Higher Derivative Gravity}},
\newblock Phys. Rev. \textbf{D77}, 126006 (2008),
\newblock \doi{10.1103/PhysRevD.77.126006},
\newblock \eprint{0712.0805}.

\bibitem{Brigante:2008gz}
M.~Brigante, H.~Liu, R.~C. Myers, S.~Shenker and S.~Yaida,
\newblock \emph{{The Viscosity Bound and Causality Violation}},
\newblock Phys. Rev. Lett. \textbf{100}, 191601 (2008),
\newblock \doi{10.1103/PhysRevLett.100.191601},
\newblock \eprint{0802.3318}.

\bibitem{Hartnoll:2016tri}
S.~A. Hartnoll, D.~M. Ramirez and J.~E. Santos,
\newblock \emph{{Entropy production, viscosity bounds and bumpy black holes}},
\newblock JHEP \textbf{03}, 170 (2016),
\newblock \doi{10.1007/JHEP03(2016)170},
\newblock \eprint{1601.02757}.

\bibitem{Alberte:2016xja}
L.~Alberte, M.~Baggioli and O.~Pujolas,
\newblock \emph{{Viscosity bound violation in holographic solids and the
  viscoelastic response}},
\newblock JHEP \textbf{07}, 074 (2016),
\newblock \doi{10.1007/JHEP07(2016)074},
\newblock \eprint{1601.03384}.

\bibitem{Baggioli:2014roa}
M.~Baggioli and O.~Pujolas,
\newblock \emph{{Electron-Phonon Interactions, Metal-Insulator Transitions, and
  Holographic Massive Gravity}},
\newblock Phys. Rev. Lett. \textbf{114}(25), 251602 (2015),
\newblock \doi{10.1103/PhysRevLett.114.251602},
\newblock \eprint{1411.1003}.

\bibitem{Alberte:2015isw}
L.~Alberte, M.~Baggioli, A.~Khmelnitsky and O.~Pujolas,
\newblock \emph{{Solid Holography and Massive Gravity}},
\newblock JHEP \textbf{02}, 114 (2016),
\newblock \doi{10.1007/JHEP02(2016)114},
\newblock \eprint{1510.09089}.

\bibitem{Andrade:2019zey}
T.~Andrade, M.~Baggioli and O.~Pujolàs,
\newblock \emph{{Viscoelastic Dynamics in Holography}}  (2019),
\newblock \eprint{1903.02859}.

\bibitem{Alberte:2017cch}
L.~Alberte, M.~Ammon, M.~Baggioli, A.~Jiménez and O.~Pujolàs,
\newblock \emph{{Black hole elasticity and gapped transverse phonons in
  holography}},
\newblock JHEP \textbf{01}, 129 (2018),
\newblock \doi{10.1007/JHEP01(2018)129},
\newblock \eprint{1708.08477}.

\bibitem{Alberte:2017oqx}
L.~Alberte, M.~Ammon, M.~Baggioli, A.~Jiménez-Alba and O.~Pujolàs,
\newblock \emph{{Holographic Phonons}}  (2017),
\newblock \eprint{1711.03100}.

\bibitem{Ammon:2019apj}
M.~Ammon, M.~Baggioli, S.~Gray and S.~Grieninger,
\newblock \emph{{Longitudinal Sound and Diffusion in Holographic Massive
  Gravity}}  (2019),
\newblock \eprint{1905.09164}.

\bibitem{Burikham:2016roo}
P.~Burikham and N.~Poovuttikul,
\newblock \emph{{Shear viscosity in holography and effective theory of
  transport without translational symmetry}},
\newblock Phys. Rev. \textbf{D94}(10), 106001 (2016),
\newblock \doi{10.1103/PhysRevD.94.106001},
\newblock \eprint{1601.04624}.

\bibitem{Ling:2016ien}
Y.~Ling, Z.-Y. Xian and Z.~Zhou,
\newblock \emph{{Holographic Shear Viscosity in Hyperscaling Violating Theories
  without Translational Invariance}},
\newblock JHEP \textbf{11}, 007 (2016),
\newblock \doi{10.1007/JHEP11(2016)007},
\newblock \eprint{1605.03879}.

\bibitem{Faulkner:2009wj}
T.~Faulkner, H.~Liu, J.~McGreevy and D.~Vegh,
\newblock \emph{{Emergent quantum criticality, Fermi surfaces, and AdS(2)}},
\newblock Phys. Rev. \textbf{D83}, 125002 (2011),
\newblock \doi{10.1103/PhysRevD.83.125002},
\newblock \eprint{0907.2694}.

\bibitem{Sachdev:2019bjn}
S.~Sachdev,
\newblock \emph{{Universal low temperature theory of charged black holes with
  AdS$_2$ horizons}},
\newblock J. Math. Phys. \textbf{60}(5), 052303 (2019),
\newblock \doi{10.1063/1.5092726},
\newblock \eprint{1902.04078}.

\bibitem{Sarosi:2017ykf}
G.~Sarosi,
\newblock \emph{{AdS$_{2}$ holography and the SYK model}},
\newblock PoS \textbf{Modave2017}, 001 (2018),
\newblock \doi{10.22323/1.323.0001},
\newblock \eprint{1711.08482}.

\bibitem{Facoetti:2019rab}
D.~Facoetti, G.~Biroli, J.~Kurchan and D.~R. Reichman,
\newblock \emph{{Classical Glasses, Black Holes, and Strange Quantum Liquids}}
  (2019),
\newblock \eprint{1906.09228}.

\bibitem{Donos:2013eha}
A.~Donos and J.~P. Gauntlett,
\newblock \emph{{Holographic Q-lattices}},
\newblock JHEP \textbf{04}, 040 (2014),
\newblock \doi{10.1007/JHEP04(2014)040},
\newblock \eprint{1311.3292}.

\bibitem{1987imsm.book.....C}
D.~{Chandler},
\newblock \emph{{Introduction to Modern Statistical Mechanics}} (1987).

\bibitem{PhysRev.86.702}
H.~B. Callen and R.~F. Greene,
\newblock \emph{On a theorem of irreversible thermodynamics},
\newblock Phys. Rev. \textbf{86}, 702 (1952),
\newblock \doi{10.1103/PhysRev.86.702}.

\bibitem{doi:10.1002/9783527638154.ch2}
\emph{The Kubo–Greenwood Linear Response Theory}, chap.~2, pp. 31--55,
\newblock John Wiley \& Sons, Ltd,
\newblock ISBN 9783527638154,
\newblock \doi{10.1002/9783527638154.ch2} (2011),
  \eprint{https://onlinelibrary.wiley.com/doi/pdf/10.1002/9783527638154.ch2}.

\bibitem{doi:10.1143/JPSJ.12.570}
R.~Kubo,
\newblock \emph{Statistical-mechanical theory of irreversible processes. i.
  general theory and simple applications to magnetic and conduction problems},
\newblock Journal of the Physical Society of Japan \textbf{12}(6), 570 (1957),
\newblock \doi{10.1143/JPSJ.12.570},
\newblock \eprint{https://doi.org/10.1143/JPSJ.12.570}.

\bibitem{Baggioli:2016oju}
M.~Baggioli and O.~Pujolas,
\newblock \emph{{On Effective Holographic Mott Insulators}},
\newblock JHEP \textbf{12}, 107 (2016),
\newblock \doi{10.1007/JHEP12(2016)107},
\newblock \eprint{1604.08915}.

\bibitem{Baggioli:2015zoa}
M.~Baggioli and M.~Goykhman,
\newblock \emph{{Phases of holographic superconductors with broken
  translational symmetry}},
\newblock JHEP \textbf{07}, 035 (2015),
\newblock \doi{10.1007/JHEP07(2015)035},
\newblock \eprint{1504.05561}.

\bibitem{1982AnPhy.144..249B}
P.~{Breitenlohner} and D.~Z. {Freedman},
\newblock \emph{{Stability in gauged extended supergravity.}},
\newblock Annals of Physics \textbf{144}, 249 (1982),
\newblock \doi{10.1016/0003-4916(82)90116-6}.

\bibitem{BREITENLOHNER1982197}
P.~Breitenlohner and D.~Z. Freedman,
\newblock \emph{Positive energy in anti-de sitter backgrounds and gauged
  extended supergravity},
\newblock Physics Letters B \textbf{115}(3), 197  (1982),
\newblock \doi{https://doi.org/10.1016/0370-2693(82)90643-8}.

\bibitem{Moroz:2009kv}
S.~Moroz,
\newblock \emph{{Below the Breitenlohner-Freedman bound in the nonrelativistic
  AdS/CFT correspondence}},
\newblock Phys. Rev. \textbf{D81}, 066002 (2010),
\newblock \doi{10.1103/PhysRevD.81.066002},
\newblock \eprint{0911.4060}.

\bibitem{Amado:2009ts}
I.~Amado, M.~Kaminski and K.~Landsteiner,
\newblock \emph{{Hydrodynamics of Holographic Superconductors}},
\newblock JHEP \textbf{05}, 021 (2009),
\newblock \doi{10.1088/1126-6708/2009/05/021},
\newblock \eprint{0903.2209}.

\bibitem{Denef:2009tp}
F.~Denef and S.~A. Hartnoll,
\newblock \emph{{Landscape of superconducting membranes}},
\newblock Phys. Rev. \textbf{D79}, 126008 (2009),
\newblock \doi{10.1103/PhysRevD.79.126008},
\newblock \eprint{0901.1160}.

\bibitem{Kaminski:2009dh}
M.~Kaminski, K.~Landsteiner, J.~Mas, J.~P. Shock and J.~Tarrio,
\newblock \emph{{Holographic Operator Mixing and Quasinormal Modes on the
  Brane}},
\newblock JHEP \textbf{02}, 021 (2010),
\newblock \doi{10.1007/JHEP02(2010)021},
\newblock \eprint{0911.3610}.

\bibitem{Ammon:2019wci}
M.~Ammon, M.~Baggioli and A.~Jimenez-Alba,
\newblock \emph{{A Unified Description of Translational Symmetry Breaking in
  Holography}}  (2019),
\newblock \eprint{1904.05785}.

\bibitem{Donos:2014cya}
A.~Donos and J.~P. Gauntlett,
\newblock \emph{{Thermoelectric DC conductivities from black hole horizons}},
\newblock JHEP \textbf{11}, 081 (2014),
\newblock \doi{10.1007/JHEP11(2014)081},
\newblock \eprint{1406.4742}.

\bibitem{Andrade:2013gsa}
T.~Andrade and B.~Withers,
\newblock \emph{{A simple holographic model of momentum relaxation}},
\newblock JHEP \textbf{1405}, 101 (2014),
\newblock \doi{10.1007/JHEP05(2014)101},
\newblock \eprint{1311.5157}.

\bibitem{kittel1976introduction}
C.~Kittel,
\newblock \emph{Introduction to solid state physics},
\newblock Wiley,
\newblock ISBN 9780471490241 (1976).

\bibitem{Baggioli:2016oqk}
M.~Baggioli and O.~Pujolas,
\newblock \emph{{On holographic disorder-driven metal-insulator transitions}},
\newblock JHEP \textbf{01}, 040 (2017),
\newblock \doi{10.1007/JHEP01(2017)040},
\newblock \eprint{1601.07897}.

\bibitem{Amoretti:2016cad}
A.~Amoretti, M.~Baggioli, N.~Magnoli and D.~Musso,
\newblock \emph{{Chasing the cuprates with dilatonic dyons}},
\newblock JHEP \textbf{06}, 113 (2016),
\newblock \doi{10.1007/JHEP06(2016)113},
\newblock \eprint{1603.03029}.

\bibitem{Baggioli:2016pia}
M.~Baggioli, B.~Goutéraux, E.~Kiritsis and W.-J. Li,
\newblock \emph{{Higher derivative corrections to incoherent metallic transport
  in holography}},
\newblock JHEP \textbf{03}, 170 (2017),
\newblock \doi{10.1007/JHEP03(2017)170},
\newblock \eprint{1612.05500}.

\bibitem{Mokhtari:2017vyz}
A.~Mokhtari, S.~A. Hosseini~Mansoori and K.~Bitaghsir~Fadafan,
\newblock \emph{{Diffusivities bounds in the presence of Weyl corrections}},
\newblock Phys. Lett. \textbf{B785}, 591 (2018),
\newblock \doi{10.1016/j.physletb.2018.09.020},
\newblock \eprint{1710.03738}.

\bibitem{Hartnoll:2012rj}
S.~A. Hartnoll and D.~M. Hofman,
\newblock \emph{{Locally Critical Resistivities from Umklapp Scattering}},
\newblock Phys. Rev. Lett. \textbf{108}, 241601 (2012),
\newblock \doi{10.1103/PhysRevLett.108.241601},
\newblock \eprint{1201.3917}.

\bibitem{Davison:2015taa}
R.~A. Davison, B.~Goutéraux and S.~A. Hartnoll,
\newblock \emph{{Incoherent transport in clean quantum critical metals}},
\newblock JHEP \textbf{10}, 112 (2015),
\newblock \doi{10.1007/JHEP10(2015)112},
\newblock \eprint{1507.07137}.

\bibitem{Amoretti:2017frz}
A.~Amoretti, D.~Areán, B.~Goutéraux and D.~Musso,
\newblock \emph{{Effective holographic theory of charge density waves}},
\newblock Phys. Rev. \textbf{D97}(8), 086017 (2018),
\newblock \doi{10.1103/PhysRevD.97.086017},
\newblock \eprint{1711.06610}.

\bibitem{Gouteraux:2018wfe}
B.~Goutéraux, N.~Jokela and A.~Pönni,
\newblock \emph{{Incoherent conductivity of holographic charge density waves}},
\newblock JHEP \textbf{07}, 004 (2018),
\newblock \doi{10.1007/JHEP07(2018)004},
\newblock \eprint{1803.03089}.

\bibitem{Donos:2018kkm}
A.~Donos, J.~P. Gauntlett, T.~Griffin and V.~Ziogas,
\newblock \emph{{Incoherent transport for phases that spontaneously break
  translations}},
\newblock JHEP \textbf{04}, 053 (2018),
\newblock \doi{10.1007/JHEP04(2018)053},
\newblock \eprint{1801.09084}.

\bibitem{Kim:2015dna}
K.-Y. Kim, K.~K. Kim and M.~Park,
\newblock \emph{{A Simple Holographic Superconductor with Momentum
  Relaxation}},
\newblock JHEP \textbf{04}, 152 (2015),
\newblock \doi{10.1007/JHEP04(2015)152},
\newblock \eprint{1501.00446}.

\bibitem{Erdmenger:2015qqa}
J.~Erdmenger, B.~Herwerth, S.~Klug, R.~Meyer and K.~Schalm,
\newblock \emph{{S-Wave Superconductivity in Anisotropic Holographic
  Insulators}},
\newblock JHEP \textbf{05}, 094 (2015),
\newblock \doi{10.1007/JHEP05(2015)094},
\newblock \eprint{1501.07615}.

\bibitem{David:2011hy}
J.~R. David, S.~Jain and S.~Thakur,
\newblock \emph{{Shear sum rules at finite chemical potential}},
\newblock JHEP \textbf{03}, 074 (2012),
\newblock \doi{10.1007/JHEP03(2012)074},
\newblock \eprint{1109.4072}.

\bibitem{David:2012cd}
J.~R. David and S.~Thakur,
\newblock \emph{{Sum rules and three point functions}},
\newblock JHEP \textbf{11}, 038 (2012),
\newblock \doi{10.1007/JHEP11(2012)038},
\newblock \eprint{1207.3912}.

\bibitem{Denef:2009kn}
F.~Denef, S.~A. Hartnoll and S.~Sachdev,
\newblock \emph{{Black hole determinants and quasinormal modes}},
\newblock Class. Quant. Grav. \textbf{27}, 125001 (2010),
\newblock \doi{10.1088/0264-9381/27/12/125001},
\newblock \eprint{0908.2657}.

\bibitem{Kokkotas:1999bd}
K.~D. Kokkotas and B.~G. Schmidt,
\newblock \emph{{Quasinormal modes of stars and black holes}},
\newblock Living Rev. Rel. \textbf{2}, 2 (1999),
\newblock \doi{10.12942/lrr-1999-2},
\newblock \eprint{gr-qc/9909058}.

\bibitem{Birmingham:2001pj}
D.~Birmingham, I.~Sachs and S.~N. Solodukhin,
\newblock \emph{{Conformal field theory interpretation of black hole
  quasinormal modes}},
\newblock Phys. Rev. Lett. \textbf{88}, 151301 (2002),
\newblock \doi{10.1103/PhysRevLett.88.151301},
\newblock \eprint{hep-th/0112055}.

\bibitem{Franz2018}
M.~Franz and M.~Rozali,
\newblock \emph{Mimicking black hole event horizons in atomic and solid-state
  systems},
\newblock Nature Reviews Materials \textbf{3}(12), 491 (2018),
\newblock \doi{10.1038/s41578-018-0058-z}.

\bibitem{Edalati:2010hk}
M.~Edalati, J.~I. Jottar and R.~G. Leigh,
\newblock \emph{{Shear Modes, Criticality and Extremal Black Holes}},
\newblock JHEP \textbf{04}, 075 (2010),
\newblock \doi{10.1007/JHEP04(2010)075},
\newblock \eprint{1001.0779}.

\bibitem{Kodama:2003kk}
H.~Kodama and A.~Ishibashi,
\newblock \emph{{Master equations for perturbations of generalized static black
  holes with charge in higher dimensions}},
\newblock Prog. Theor. Phys. \textbf{111}, 29 (2004),
\newblock \doi{10.1143/PTP.111.29},
\newblock \eprint{hep-th/0308128}.

\end{thebibliography}


==> solutions.tex <==

\Extrachap{Solutions}

\section*{Problems of Chapter~\ref{intro}}

\begin{sol}{prob1}
The solution\index{problems}\index{solutions} is revealed here.
\end{sol}


\begin{sol}{prob2}
\textbf{Problem Heading}\\
(a) The solution of first part is revealed here.\\
(b) The solution of second part is revealed here.
\end{sol}


